PlanningVis: A Visual Analytics Approach to Production Planning in Smart Factories

Production planning in the manufacturing industry is crucial for fully utilizing factory resources (e.g., machines, raw materials and workers) and reducing costs. With the advent of industry 4.0, plenty of data recording the status of factory resources have been collected and further involved in production planning, which brings an unprecedented opportunity to understand, evaluate and adjust complex production plans through a data-driven approach. However, developing a systematic analytics approach for production planning is challenging due to the large volume of production data, the complex dependency between products, and unexpected changes in the market and the plant. Previous studies only provide summarized results and fail to show details for comparative analysis of production plans. Besides, the rapid adjustment to the plan in the case of an unanticipated incident is also not supported. In this paper, we propose PlanningVis, a visual analytics system to support the exploration and comparison of production plans with three levels of details: a plan overview presenting the overall difference between plans, a product view visualizing various properties of individual products, and a production detail view displaying the product dependency and the daily production details in related factories. By integrating an automatic planning algorithm with interactive visual explorations, PlanningVis can facilitate the efficient optimization of daily production planning as well as support a quick response to unanticipated incidents in manufacturing. Two case studies with real-world data and carefully designed interviews with domain experts demonstrate the effectiveness and usability of PlanningVis.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> src/algorithm_detail.tex <==
The production planning problem is inherently a multi-objective optimization problem. Therefore, we first describe our problem as such a mathematical problem. As mentioned, the objectives we concentrated on are the four performance indicators suggested by domain experts. The first objective is to minimize the order delay rate:
\begin{equation}
\label{eqn:order_delay}
    A_{delay} = 
    % \min
    % \left\{
        \sum_{i \in I_D} \sum_{t \in T} \frac{m_{i, t}}{D_{i, t} + 1}
    % \right\},
\end{equation}
where $I_D$ is the products with demand, \modified{$T$ represents the dates the production plan targets at,} $m_{i, t}$ means the amount of order delayed, and $D_{i, t}$ denotes the total order demand. \modified{The timestep of the algorithm is one day.} The denominator is added by one to avoid the error caused when the demand is 0. 
% production cost
The second objective, minimizing the production cost, is formulated as follows:
\begin{equation}
\label{eqn:production_cost}
    A_{cost_p} = 
    % \min
    % \left\{
        \sum_{i \in I_{AI}} \sum_{p \in P_i} PC_{i,p} \cdot
        \left(
            \sum_{t \in T} \hat{x}_{i, p, t}
        \right)
    % \right\},
\end{equation}
where $I_{AI}$ encodes the products whose production will consume other products or raw materials, $P_i$ denotes the plants which can produce product $i$, $PC_{i, p}$ represents the unit production cost, and $\hat{x}_{i, p, t}$ denotes the planned production output. 
% inventory cost
Minimizing the inventory cost is the third objective:
\begin{equation}
\label{eqn:inventory_cost}
    A_{cost_i} = 
    \sum_{i \in I_{AI}} \sum_{p \in P_i} HC_{i, p} \cdot \sum_{t \in T} inv_{i, p, t}
    + \sum_{i \in I_{AI}} \sum_{p \in P_i} HC_{i, p} \cdot PT_{i, p} \cdot \sum_{t \in T} \hat{x}_{i, p, t},
\end{equation}
where $HC_{i, p}$ indicates the unit inventory cost, \modified{$inv_{i, p, t}$ denotes the inventory of the product at the end of a day, and $PT_{i, p}$ denotes the processing cycle of the product}. From Eqn.~\ref{eqn:inventory_cost}, we can see besides the inventory cost of finished products, the cost also includes products which are under processing. The second term in Eqn.~\ref{eqn:inventory_cost} is added to meet the requirement mentioned by domain experts.

% smoothing rate of production capacity use
The last objective is to minimize the weekly smoothing rate of production capacity use. Eqn.~\ref{eqn:smoothing_rate} is used to compute the smoothing rate of a capacity set $c$ in week $T$:
\begin{equation}
\label{eqn:smoothing_rate}
    A_{smooth_{c, T}} = 
    % \min
    % \left\{
        \frac{|\sum_{t \in T} \sum_{i \in I_{p, c}} U_{i, p, c} \cdot \hat{x}_{i, p, t} - \sum_{t \in \overline{T - 1}} \sum_{i \in I_{p, c}} U_{i, p, c} \cdot \hat{x}_{i, p, t}|}
        {\sum_{t \in \overline{T - 1}} \sum_{i \in I_{p, c}} U_{i, p, c} \cdot \hat{x}_{i, p, t} + 1}.
    % \right\}
\end{equation}
Here, $\overline{T - 1}$ means the week before week T and $U_{i, p, c}$ represents unit production capacity. The objective is got by averaging the smoothing rate of all the capacity sets. 

Then, we employ the weighted sum model (WSM) \cite{triantaphyllou2000multi} to address the multi-objective production planning problem:
\begin{equation}
\label{eqn:score}
    WSM_{score} ^* = w_1 A_{delay}+w_2 A_{cost_p}+w_3 A_{cost_i}+ w_4 A_{smooth_{c, T}} 
\end{equation}
The optimized plan is reached by minimize $WSM_{score} ^*$, and the decision variables are $\hat{x}_{i, p, t}$. The weights $w_j$ are predefined by domain experts according to the importance of the four performance indicators. 

The optimization model also contains a huge number of constraints which can be grouped into more than 20 categories. For example, the maximum production output of the product is constrained by the production capacity of the factory, as illustrated in the following inequality:
\begin{equation}
    \sum_{i \in I_{p, c}} U_{i, p, c} \cdot \hat{x}_{i, p, t} \le CAP_{p, t, c}, 
    \forall p \in P, \forall t \in T, \forall c \in C,
\end{equation}
where $CAP_{p, t, c}$ denotes the maximum production capacity available. Due to limited space, other types of constraints will not be described in detail.
% We then exploit a Lagrangian relaxation approach \cite{diaby1992lagrangean} to convert the constraint of production capacity to punishment on the objective. 

% the algorithm used
The optimized plan described in Eqn.~\ref{eqn:score} can be solved by integer programming. 
However, directly employing integer programming to solve such a large scale production planning problem is too time consuming. Therefore, in this paper, we adopt a hybrid production planning algorithm which combines linear programming \cite{shapiro1993mathematical} and heuristic algorithms \cite{li2007heuristic}. It is adapted from an approach proposed by Sahling et al. \cite{sahling2009solving} 

% mathematical programming
% Linear programming \cite{shapiro1993mathematical} is a widely utilized method for multi-objective decision problems, which can produces a near optimal solution.
% However, since the variables in production planning are integers, the solution of linear programming is not applicable.
% To bridge the gap, a greedy heuristic approach \cite{sahling2009solving} is introduced to repair non-integer values to integers under the give constraints. 
% We repeatedly repair non-integer variables and solve the linear programming model until all the variables are integers.
% and the problem inherently has similar business logic, such as production constraints and objectives. 
% Among the multiple objectives in production planning, we concentrate on four important ones suggested by domain experts. 
% order delay rate

==> temp.tex <==
Production planning in the manufacturing industry is crucial for fully utilizing factory resources (e.g., machines, raw materials, product components and workers) and reducing costs. With the advent of industry 4.0, plenty of data recording the status of factory resources have been collected and further involved in production planning, which brings an unprecedented opportunity to understand, evaluate and adjust complex production plans through a data-driven approach. However, developing a systematic analytics approach for production planning is often challenging due to the large volume of production data, the complex dependence between products, and unexpected changes in the market demand, material supplies and the production process. Previous studies only provide summarized results and fail to show details for comparative analysis of production plans. Besides, the rapid adjustment to the plan in the case of an unanticipated incident is also not supported. In this paper, we propose PlanningVis, a visual analytics system to support the exploration and comparison of production plans with three levels of details: a plan overview presenting the overall difference between plans, a product view visualizing various properties of individual products, and a production detail view displaying the product dependency, the daily production output and production capacity usage in related factories. By integrating an automatic planning algorithm with interactive visual explorations, PlanningVis is able to facilitate efficient optimization of daily production planning as well as supporting a quick response to unanticipated incidents in manufacturing. Two case studies with real-world data and carefully designed interviews with domain experts from a world-leading manufacturing company demonstrate the effectiveness and usability of PlanningVis. 
